Predictive and Robust Robot Assistance for Sequential Manipulation

This paper presents a novel concept to support physically impaired humans in daily object manipulation tasks with a robot. Given a user's manipulation sequence, we propose a predictive model that uniquely casts the user's sequential behavior as well as a robot support intervention into a hierarchical multi-objective optimization problem. A major contribution is the prediction formulation, which allows to consider several different future paths concurrently. The second contribution is the encoding of a general notion of constancy constraints, which allows to consider dependencies between consecutive or far apart keyframes (in time or space) of a sequential task. We perform numerical studies, simulations and robot experiments to analyse and evaluate the proposed method in several table top tasks where a robot supports impaired users by predicting their posture and proactively re-arranging objects.

==> sections/Exp_results.tex <==

\subsection{Demonstrators - simulation}

\subsubsection{Use case long linear prediction}
For example~\cref{fig:sequences}.
\theo{Optimal placement of objects for a sequence of tasks}


\subsubsection{Use case tree-based prediction to consider uncertainty}
For example~\cref{fig:tree_sequence}.\\
\theo{Placement/orienting a mug with a handle, if the liquid is hot then handle (precision-grasp) will be used, if the liquid is cold the power grasps might be preferred}.
\theo{Maybe show these in simulation: Variations of reaching with different end-effectors, objects, affordances}
\theo{Maybe show these in simulation: Variations of postures based on static effort}


\subsubsection{Long horizon intervention - hardware}

\theo{Evaluate REBA (using Xsens) of a keyframe far in the future, but intervene with the robot now.}

